Modularizing while Training: A New Paradigm for Modularizing DNN Models

Deep neural network (DNN) models have become increasingly crucial components in intelligent software systems. However, training a DNN model is typically expensive in terms of both time and money. To address this issue, researchers have recently focused on reusing existing DNN models - borrowing the idea of code reuse in software engineering. However, reusing an entire model could cause extra overhead or inherits the weakness from the undesired functionalities. Hence, existing work proposes to decompose an already trained model into modules, i.e., modularizing-after-training, and enable module reuse. Since trained models are not built for modularization, modularizing-after-training incurs huge overhead and model accuracy loss. In this paper, we propose a novel approach that incorporates modularization into the model training process, i.e., modularizing-while-training (MwT). We train a model to be structurally modular through two loss functions that optimize intra-module cohesion and inter-module coupling. We have implemented the proposed approach for modularizing Convolutional Neural Network (CNN) models in this work. The evaluation results on representative models demonstrate that MwT outperforms the state-of-the-art approach. Specifically, the accuracy loss caused by MwT is only 1.13 percentage points, which is 1.76 percentage points less than that of the baseline. The kernel retention rate of the modules generated by MwT is only 14.58%, with a reduction of 74.31% over the state-of-the-art approach. Furthermore, the total time cost required for training and modularizing is only 108 minutes, half of the baseline.

==> motivation.tex <==
\subsection{Motivation}







Although the existing two types of approaches have made some progress in DNN modularization, they both belong to the paradigm of \textit{modularizing after training}.
The lack of consideration for modularization during the training process has led to three main limitations for modularizing after training.


First, during training, the model predicts each sample using all weights, and most neurons are activated. Consequently, for each class, while there may be variations in the relevance of different weights and neurons, the majority of them are utilized in prediction, which could lead to a high weight retention rate. 
For instance, the module generated by ~\cite{fse2020modularity} retains 76.21\% of the weights, and the module produced by ~\cite{nnmodularity2022icse} retains 81.41\% of the neurons. CNNSplitter~\cite{qi2022patching} achieves better performance, but its resulting module still retains 56.76\% of the convolution kernels.

Second, the training process cannot explicitly identify relevant weights or neurons. Therefore, modularization needs to identify relevant weights after the training process. However, the post-process may result in significant time consumption due to the huge search space~\cite{qi2022patching} or may result in a high weight retention rate due to inaccurate identification caused by inappropriate evaluation metrics for relevance~\cite{ReMos}. 

Last, a module can be perceived as an altered model that removes the irrelevant weights or sets the irrelevant neurons and weights to zero. Since the original model has not learned to predict using only relevant neurons and weights, the altered model (i.e., module) may not perform well. That is, modularization could cause much loss of accuracy~\cite{nnmodularity2022icse,qi2022patching}.
For instance, the average loss of accuracy caused by CNNSplitter~\cite{qi2022patching} is 2.89\%.

To this end, we propose a new paradigm of \textit{modularizing while training} for DNN modularization, which can consider modularization during the training, thus addressing the above issues.
